Human Attention in Visual Question Answering: Do Humans and Deep Networks Look at the Same Regions?

We conduct large-scale studies on `human attention' in Visual Question Answering (VQA) to understand where humans choose to look to answer questions about images. We design and test multiple game-inspired novel attention-annotation interfaces that require the subject to sharpen regions of a blurred image to answer a question. Thus, we introduce the VQA-HAT (Human ATtention) dataset. We evaluate attention maps generated by state-of-the-art VQA models against human attention both qualitatively (via visualizations) and quantitatively (via rank-order correlation). Overall, our experiments show that current attention models in VQA do not seem to be looking at the same regions as humans.

==> sections/abstract-extended.tex <==
It helps to pay attention.
Humans have the ability to quickly perceive a scene by selectively attending to parts of the image instead of processing the whole scene in its entirety \cite{rensink_vc2000}.
% This ability to intelligently pick where to look is task-specific \cite{land_vr05} and helps reduce problem complexity, as fixations can center on regions of interest and ignore background clutter.
Inspired by human attention, a recent trend in computer vision and deep learning is to build computational models of attention.
Given an input signal, these models learn to attend to parts of it for further processing and have been successfully applied in machine translation \cite{bahdanau_iclr15,firat_arxiv16}, object recognition \cite{ba_iclr15,mnih_arxiv14,sermanet_arxiv14}, image captioning \cite{xu_arxiv15,cho_arxiv15} and visual question answering \cite{yang_arxiv15,lu_arxiv16,hxu_arxiv15,xiong_arxiv16}.

In this work, we study attention for the task of Visual Question Answering (VQA).
Unlike image captioning, where a coarse understanding of an image is often sufficient for producing generic descriptions \cite{devlin_arxiv15}, visual questions selectively target different areas of an image including background details and underlying context.
This suggests that a VQA model may benefit from an explicit or implicit attention mechanism to answer a question correctly.

In this work, we are interested in the following questions:
1) Which image regions do humans choose to look at in order to answer questions about images?
2) Do deep VQA models with attention mechanisms attend to the same regions as humans?

We design and conduct studies to collect ``human attention maps".
\figref{fig:teaser} shows human attention maps on the same image for two different questions.
When asked `What type is the surface?', humans choose to look at the floor, while attention for `Which game is being played?' is concentrated around the player and racket.

\begin{figure}[t]
    \includegraphics[width=1\linewidth]{figures/teaser.png}
    \caption{Different human attention regions based on question, with 80\% probability mass bounding boxes.}
    \label{fig:teaser}
\end{figure}

\begin{figure*}[ht]
  \centering
  \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=1\linewidth]{figures/human_blurred_maps_qa_small_1.png}
    \caption{}
  \end{subfigure}
  \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=1\linewidth]{figures/human_blurred_maps_qa_small_2.png}
    \caption{}
  \end{subfigure}
  \begin{subfigure}[b]{0.32\textwidth}
    \includegraphics[width=1\linewidth]{figures/human_blurred_maps_qa_small_3.png}
    \caption{}
  \end{subfigure}
  \caption{
    (a-c): Column 1 shows deblurred image, and column 2 shows human attention map.}
  \label{fig:human_maps}
\end{figure*}

% In order to perform large-scale studies on hundreds of thousands of images and questions, we conduct human studies on Amazon Mechanical Turk (AMT). % that require subjects to `deblur' regions.

These human attention maps can be used both for evaluating machine-generated attention maps and for explicitly training attention-based models.
% We also highlight an important distinction between our study and several other task-independent studies on saliency \cite{Jiang2015, Judd2009}.

\noindent \textbf{Contributions.}
% Concretely, our contributions are twofold.
First, we design and test multiple game-inspired novel interfaces for collecting human attention maps of where humans choose to look to answer questions from the large-scale VQA dataset \cite{antol_iccv15}; this VQA-HAT (Human ATtention) dataset will be released publicly.
% We experiment with multiple variants of our attention annotation interface that requires the subject to sharpen regions of a blurred image to answer visual questions accurately.
% Post careful analysis of our attention annotation interface, we collect human attention maps on a subset of the VQA dataset \cite{antol_iccv15}, which will be made publicly available.
Second, we perform qualitative and quantitative comparison of the maps generated by state-of-the-art attention-based VQA models \cite{yang_arxiv15,lu_arxiv16} and a task-independent saliency baseline \cite{judd_iccv09} against our human attention maps through visualizations and rank-order correlation.
% Second, we perform qualitative and quantitative comparison of the maps generated by state-of-the-art attention-based VQA models and a task-independent saliency baseline against our human attention maps through visualizations and rank-order correlation.
We find that machine-generated attention maps from the most accurate VQA model have a mean rank-correlation of 0.26 with human attention maps, which is worse than task-independent saliency maps that have a mean rank-correlation of 0.49.
It is well understood that task-independent saliency maps have a `center bias'~\cite{tatler_jov07,judd_iccv09}.
After we control for this center bias in our human attention maps, we find that the correlation of task-independent saliency is poor (as expected), while trends for machine-generated VQA-attention maps remain the same (which is promising).

Our basic interface design consists of a ``deblurring" exercise for answering visual questions.
Specifically, we present subjects with a blurred image and a question about the image, and ask subjects to sharpen regions of the image to answer the question correctly, in a smooth, click-and-drag, `coloring' motion with the mouse.
The sharpening is gradual: successively scrubbing the same region progressively sharpens it.

Our interface starts by showing a low-resolution blurry version of the image.
This is to convey a partial `holistic' understanding of the scene to the subjects so they may intelligently choose which regions to sharpen.
Gradual sharpening with strokes was aimed to capture initial exploration as they tried to get a better sense of the scene, and eventually focussed sharpening to answer the question.

In order to quantitatively evaluate the attention annotation interfaces we experimented with, we conducted a second human study where (a second set of) subjects where shown the attention-sharpened images generated from each of the attention interfaces from the first experiment and asked to answer the question.
The intuition behind this experiment is that if the attention map revealed too little information, this second set of subjects would answer the question incorrectly. Since the payments structure on AMT encourage completing tasks as quickly as possible, this implicitly incentivizes subjects to deblur as few regions as possible, and our human study shows that humans can still answer questions.
Thus, overall we achieve a balance between highlighting too little or too much.

Overall, we collected human attention maps for 58475 train (out of 248349 total) and 1374 val (out of 121512 total) question-image pairs in the VQA dataset respectively.
\figref{fig:human_maps} shows examples of collected human attention heatmaps overlayed on original images.

% We introduce and release the VQA-HAT dataset.
% Using the interface that gives highest human accuracy, we collect a human attention maps dataset which will be made publicly available.
The VQA-HAT dataset can be used to evaluate attention maps generated in an unsupervised manner by attention-based VQA models, or to explicitly train models with attention supervision for VQA.
We quantify whether current attention-based VQA models are `looking' at the same regions of the image as humans do to produce an answer.

\noindent \textbf{Necessary vs Sufficient Maps.} Are human attention maps `necessary' and/or `sufficient'?
If regions highlighted by the human attention maps are sufficient to answer the question accurately, then so is any region that is a superset.
For example, if attention mass is concentrated on a `cat' for `What animal is present in the picture?', then an attention map that assigns weights to any arbitrary-sized region that includes the `cat' is sufficient as well.
On the contrary, a \emph{necessary} and sufficient attention map would be the smallest visual region sufficient for answering the question accurately.
It is an ill-posed problem to define a necessary attention map in the space of pixels; random pixels can be blacked out and chances are that humans would still be able to answer the question given the resulting subset attention map.
% In pixel space, human attention maps will always be approximate.
% However, it may be possible to work with a more constrained framework, for example hard attention blobs or bounding boxes, and define necessary and sufficient within that framework.
% Ideally, human attention maps should be necessary and sufficient in the semantic space and determining the right semantic representation is an open research problem.
% This distinction between pixel and semantic representation of necessary and sufficient human attention maps is important because it makes sense to train a model to emulate the best machines, i.e. humans, so attention maps that are semantically necessary and sufficient for humans would make for the `best' ground truth.
Our work thus poses an interesting question for future work -- what is the right \emph{semantic} space in which it is meaningful to talk about necessary and sufficient attention maps for humans?

\textbf{Acknowledgements.} We thank Jiasen Lu and Ramakrishna Vedantam for helpful suggestions and discussions.
This work was supported in part by the following:
National Science Foundation CAREER awards to DB and DP,
Army Research Office YIP awards to DB and DP,
ICTAS Junior Faculty awards to DB and DP,
Army Research Lab grant W911NF-15-2-0080 to DP and DB,
Office of Naval Research grant N00014-14-1-0679 to DB,
Paul G. Allen Family Foundation Allen Distinguished Investigator award to DP,
Google Faculty Research award to DP and DB,
AWS in Education Research grant to DB, and NVIDIA GPU donation to DB.


==> sections/conclusion.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % \vspace{\sectionReduceBot}
% \section{Conclusion}
% \label{sec:conclusion}
% % \vspace{\sectionReduceBot}
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% We introduce and collect a human attention maps dataset for VQA.
% % Using the interface that gives highest human accuracy, we collect a human attention maps dataset which will be made publicly available.
% This dataset can be used to evaluate attention maps generated in an unsupervised manner by attention-based VQA models, or to explicitly train models with attention supervision for VQA.
% We quantify whether current attention-based VQA models are `looking' at the same regions of the image as humans do to produce an answer.

